Towards Autonomous Navigation in Endovascular Interventions

Cardiovascular diseases remain the leading cause of global mortality, with minimally invasive treatment options offered through endovascular interventions. However, the precision and adaptability of current robotic systems for endovascular navigation are limited by heuristic control, low autonomy, and the absence of haptic feedback. This thesis presents an integrated AI-driven framework for autonomous guidewire navigation in complex vascular environments, addressing key challenges in data availability, simulation fidelity, and navigational accuracy. A high-fidelity, real-time simulation platform, CathSim, is introduced for reinforcement learning based catheter navigation, featuring anatomically accurate vascular models and contact dynamics. Building on CathSim, the Expert Navigation Network is developed, a policy that fuses visual, kinematic, and force feedback for autonomous tool control. To mitigate data scarcity, the open-source, bi-planar fluoroscopic dataset Guide3D is proposed, comprising more than 8,700 annotated images for 3D guidewire reconstruction. Finally, SplineFormer, a transformer-based model, is introduced to directly predict guidewire geometry as continuous B-spline parameters, enabling interpretable, real-time navigation. The findings show that combining high-fidelity simulation, multimodal sensory fusion, and geometric modelling substantially improves autonomous endovascular navigation and supports safer, more precise minimally invasive procedures.

==> chapters/ch3_cathsim/tables/environments_1.tex <==
\begin{table*}[t]
\caption{Comparison of CathSim, SofaGym, and LapGym Simulator Environments}
\begin{center}
\begin{tabular}{l c c c c c c}
\toprule
Simulator & Focus Area & Physics Engine  & Gym/Gymnasium & Deformable Objects & Domain Randomization  \\
\midrule
SofaGym~\cite{schegg2023sofagym} & General SOFA Environments & SOFA~\cite{faure:hal-00681539} & Gym & FEM / Mass-Spring & \xmark \\
LapGym~\cite{scheikl2023lapgym} & Laparoscopic Surgery & SOFA~\cite{faure:hal-00681539} & Gym & FEM / Mass-Spring & \xmark \\
\textbf{CathSim} (ours) & Endovascular Navigation & MuJoCo~\cite{mujoco} & Gymnasium & Mass-Spring & \cmark \\
\bottomrule
\end{tabular}
\label{tab:comparison_simulators}
\end{center}
\end{table*}


==> chapters/ch3_cathsim/tables/environments_2.tex <==
\begin{table*}[t]
\caption{Comparison of CathSim, SofaGym, and LapGym Simulator Environments}
\begin{center}
\begin{tabular}{l c c c c c c}
\toprule
Simulator & Focus Area & Physics Engine  & Gym/Gymnasium & Deformable Objects & Domain Randomization  \\
\midrule
SofaGym~\cite{schegg2023sofagym} & General SOFA Environments & SOFA~\cite{faure:hal-00681539} & Gym & FEM / Mass-Spring & \xmark \\
LapGym~\cite{scheikl2023lapgym} & Laparoscopic Surgery & SOFA~\cite{faure:hal-00681539} & Gym & FEM / Mass-Spring & \xmark \\
\textbf{CathSim} (ours) & Endovascular Navigation & MuJoCo~\cite{mujoco} & Gymnasium & Mass-Spring & \cmark \\
\bottomrule
\end{tabular}
\label{tab:comparison_simulators}
\end{center}
\end{table*}


==> chapters/ch3_cathsim/tables/rl_initial_results.tex <==
	\begin{table}[ht]
		\centering
		\caption{Results Summary}\label{ch3tab:cathsim_initial_results}
		\begin{tabular}{
l 
l 
S[table-format=3(2)] 
S[table-format=3(2)] 
S[table-format=.3(.3)] 
S[table-format=.3(.3)] 
S[table-format=.3(.3)] 
S[table-format=.3(.3)] 
S[table-format=3] 
S[table-format=3]
}
			\toprule
			 &  & \multicolumn{2}{c}{\thead{Reward}}  & \multicolumn{2}{c}{\thead{Mean Force $(N\downarrow)$}} & \multicolumn{2}{c}{\thead{Max Force $(N\downarrow)$}} & \multicolumn{2}{c}{Success~\%}                                                                                  \\
			\cmidrule{3-10}
			\thead{Aorta}						 & \thead{Observation}                                 & {BCA}             & {LCCA}                                                 & {BCA}                                                 & {LCCA}                         & {BCA}                  & {LCCA}                 & {BCA}         & {LCCA}       \\
			\midrule
			\multirow{6}{*}{Type-I}
			                                             & PPO-Internal                     & -70(28)           & -154(66)                                               & 0.011(0.021)                                          & 0.008(0.015)                   & 0.121(0.095)           & 0.123(0.089)           & 53            & 07           \\
			                                             & SAC-Internal                     & -54(36)           & -158(83)                                               & 0.007(0.014)                                          & 0.006(0.015)                   & 0.059(0.047)           & 0.095(0.039)           & 77            & 07           \\
			                                             & PPO-Image                        & -65(52)           & \bfseries -140(96)                                     & \bfseries 0.005(0.007)                                & 0.007(0.016)                   & \bfseries 0.048(0.020) & 0.076(0.059)           & 83            & \bfseries 37 \\
			                                             & SAC-Image                        & -391(157)         & -196(5)                                                & 0.024(0.035)                                          & \bfseries 0.003(0.003)         & 0.258(0.094)           & \bfseries 0.059(0.028) & 00            & 00           \\
			                                             & PPO-Sequential                   & \bfseries -57(36) & -336(55)                                               & 0.006(0.009)                                          & 0.010(0.015)                   & 0.045(0.022)           & 0.094(0.036)           & \bfseries  97  & 00           \\
			                                             & SAC-Sequential                   & -200(20)          & -227(12)                                               & 0.003(0.003)                                          & 0.003(0.003)                   & 0.043(0.009)           & 0.061(0.022)           & 00            & 00           \\
			\midrule                                                                                                                                                                                                            
			\multirow{6}{*}{Type-II}
			                                             & PPO-Internal                     & -52(48)           & -22(30)                                                & 0.016(0.023)                                          & 0.011(0.015)                   & 0.118(0.103)           & 0.068(0.040)           & 50            & 87           \\
			                                             & SAC-Internal                     & \bfseries 0(0)    & -67(30)                                                & 0.014(0.010)                                          & 0.010(0.016)                   & \bfseries 0.030(0.007) & 0.121(0.044)           & \bfseries  100 & 27           \\
			                                             & PPO-Image                        & -20(47)           & \bfseries -8(10)                                       & 0.017(0.025)                                          & 0.015(0.022)                   & 0.046(0.047)           & 0.066(0.054)           & 87            & \bfseries 97 \\
			                                             & SAC-Image                        & -68(91)           & -54(7)                                                 & \bfseries 0.004(0.005)                                & \bfseries 0.005(0.005)         & 0.042(0.013)           & \bfseries  0.050(0.008) & 73            & 03           \\
			                                             & PPO-Sequential                   & -47(49)           & -80(92)                                                & 0.011(0.017)                                          & 0.011(0.018)                   & 0.068(0.059)           & 0.066(0.050)           & 57            & 67           \\
			                                             & SAC-Sequential                   & -99(18)           & -85(15)                                                & 0.005(0.007)                                          & 0.006(0.008)                   & 0.055(0.017)           & 0.100(0.023)           & 03            & 00           \\
			\bottomrule
		\end{tabular}
\end{table}

% \clearpage
% \begin{landscape}
% 	\hspace*{\fill}
% 	\vspace*{\fill}
% 	\begin{table}[htbp]
% 		\centering
% 		\caption{Results Summary}
% 		\vspace{0.3cm}
% 		\label{tab:cathsim-initial-results}
% 		\begin{tabular}{@{}llrrrrrrrrrrr@{}}\toprule
% 			\multicolumn{1}{c}{\multirow{2}{*}{Aorta}} & \multicolumn{1}{c}{\multirow{2}{*}{Observation}} & \multicolumn{2}{c}{Reward} & \multicolumn{2}{c}{Mean Force~$\mathrm{(N)}~\downarrow$} & \multicolumn{2}{c}{Max Force~$\mathrm{(N)}~\downarrow$} & \multicolumn{2}{c}{Success~\%}                                                                                                                \\
% 			\cmidrule{3-4} \cmidrule{5-6} \cmidrule{7-8} \cmidrule{9-10}
% 			                                           &                                                  & \multicolumn{1}{c}{BCA}    & \multicolumn{1}{c}{LCCA}                                 & \multicolumn{1}{c}{BCA}                                 & \multicolumn{1}{c}{LCCA}       & \multicolumn{1}{c}{BCA}    & \multicolumn{1}{c}{LCCA}   & \multicolumn{1}{c}{BCA} & \multicolumn{1}{c}{LCCA} \\
% 			\midrule
% 			\multirow{6}{*}{Type-I}
% 			                                           & PPO-Internal                                     & $-70  \pm 28$              & $-154 \pm 66$                                            & $0.011 \pm 0.021$                                       & $0.008 \pm 0.015$              & $0.121 \pm 0.095$          & $0.123 \pm 0.089$          & $53$                    & $07$                     \\
% 			                                           & SAC-Internal                                     & $-54  \pm 36$              & $-158 \pm 83$                                            & $0.007 \pm 0.014$                                       & $0.006 \pm 0.015$              & $0.059 \pm 0.047$          & $0.095 \pm 0.039$          & $77$                    & $07$                     \\
% 			                                           & PPO-Image                                        & $ -65 \pm 52$              & $\textbf{-140} \pm 96$                                   & $\textbf{0.005} \pm 0.007$                              & $0.007 \pm 0.016$              & $\textbf{0.048} \pm 0.020$ & $0.076 \pm 0.059$          & $83$                    & $\textbf{37}$            \\
% 			                                           & SAC-Image                                        & $-391 \pm 157$             & $ -196 \pm 5$                                            & $0.024 \pm 0.035$                                       & $\textbf{0.003} \pm 0.003$     & $0.258 \pm 0.094$          & $\textbf{0.059} \pm 0.028$ & $00$                    & $00$                     \\
% 			                                           & PPO-Sequential                                   & $\textbf{-57} \pm 36$      & $-336 \pm 55$                                            & $0.006 \pm 0.009$                                       & $0.010 \pm 0.015$              & $0.045 \pm 0.022$          & $0.094 \pm 0.036$          & $\textbf{97}$           & $00$                     \\
% 			                                           & SAC-Sequential                                   & $-200 \pm 20$              & $-227 \pm 12$                                            & $0.003 \pm 0.003$                                       & $0.003 \pm 0.003$              & $0.043 \pm 0.009$          & $0.061 \pm 0.022$          & $00$                    & $00$                     \\
% 			\midrule
% 			\multirow{6}{*}{Type-II}
% 			                                           & PPO-Internal                                     & $-52 \pm 48$               & $-22 \pm 30$                                             & $0.016 \pm 0.023$                                       & $0.011 \pm 0.015$              & $0.118 \pm 0.103$          & $0.068 \pm 0.040$          & $50$                    & $87$                     \\
% 			                                           & SAC-Internal                                     & $   \textbf{0} \pm 0$      & $-67 \pm 30$                                             & $0.014 \pm 0.010$                                       & $0.010 \pm 0.016$              & $\textbf{0.030} \pm 0.007$ & $0.121 \pm 0.044$          & $\textbf{100}$          & $27$                     \\
% 			                                           & PPO-Image                                        & $-20 \pm 47$               & $ \textbf{-8} \pm 10$                                    & $0.017 \pm 0.025$                                       & $0.015 \pm 0.022$              & $0.046 \pm 0.047$          & $0.066 \pm 0.054$          & $87$                    & $\textbf{97}$            \\
% 			                                           & SAC-Image                                        & $-68 \pm 91$               & $-54 \pm 7$                                              & $\textbf{0.004} \pm 0.005$                              & $\textbf{0.005} \pm 0.005$     & $0.042 \pm 0.013$          & $\textbf{0.050} \pm 0.008$ & $73$                    & $03$                     \\
% 			                                           & PPO-Sequential                                   & $-47 \pm 49$               & $-80 \pm 92$                                             & $0.011 \pm 0.017$                                       & $0.011 \pm 0.018$              & $0.068 \pm 0.059$          & $0.066 \pm 0.050$          & $57$                    & $67$                     \\
% 			                                           & SAC-Sequential                                   & $-99 \pm 18$               & $-85 \pm 15$                                             & $0.005 \pm 0.007$                                       & $0.006 \pm 0.008$              & $0.055 \pm 0.017$          & $0.100 \pm 0.023$          & $03$                    & $00$                     \\
% 			\bottomrule
% 		\end{tabular}
% 	\end{table}
% 	\hspace*{\fill}
% 	\vspace*{\fill}
% \end{landscape}
% \clearpage


==> chapters/ch4_expert_navigation/sections/1_intro.tex <==
\section{Introduction}

Endovascular interventions are widely employed for diagnosing and treating various vascular diseases. These procedures utilize flexible instruments such as guidewires and catheters, which are introduced into the body through small incisions and guided manually through the vascular system to reach target regions, including the heart or brain~\autocite{wamala2017use}. Navigation of endovascular tools accounts for approximately 70\% of the total intervention time and is applied in the treatment of conditions such as Peripheral Artery Disease (PAD), aneurysms, and stenosis~\autocite{padsalgikar2017cardiovascular}. Endovascular techniques offer significant advantages over traditional open surgery, including reduced recovery times, lower levels of pain and scarring, and a decreased risk of complications~\autocite{wamala2017use}. Despite these benefits, surgeons must rely on monoplanar X-ray imaging for visual feedback, which introduces operational challenges. Consequently, prolonged exposure to occupational hazards such as radiation and orthopaedic strain is common. Moreover, manual manipulation of guidewires and catheters requires advanced surgical expertise, while the absence of haptic feedback and limited visualization hinder precision during these procedures~\autocite{omisore2018tbcas}.

In response to these limitations, robotic systems have been developed to assist surgeons during endovascular procedures~\autocite{kundrat2021mr}. These systems allow for remote operation, thereby reducing direct exposure to intraoperative hazards~\autocite{mahmud2016feasibility}. However, most current systems operate on a follower-leader (master-slave) architecture, in which the surgeon retains full control of navigation~\autocite{puschel2022robot}. Furthermore, manually operated robotic systems impose high cognitive demands and are frequently associated with longer procedural durations when compared to traditional non-robotic techniques~\autocite{jara2020complications}. As such, the development of autonomous solutions for endovascular tasks has emerged as a critical area of research.

Autonomous catheterization, an evolving challenge within the \gls{machine learning} domain, has motivated the introduction of an expert trajectory solution as a robust baseline. Expert trajectories encapsulate the complexity of surgical procedures and provide a structured framework for training autonomous systems~\autocite{kiran2021deep}. Through \gls{imitation learning}, these systems are able to replicate expert behaviour with high fidelity, thereby accelerating the transition from novice to proficient interventionist. \textit{CathSim} offers a dynamic and safe simulation environment that enables autonomous agents to iteratively refine their performance through expert-guided actions~\autocite{li20223d}. Experimental results have shown that expert-guided learning in simulation substantially improves downstream \gls{machine learning} tasks related to autonomous catheterization, including \gls{imitation learning} and force prediction. This contribution includes an expert trajectory network along with a novel set of evaluation metrics designed to assess its performance in such tasks. These advancements aim to extend the capabilities of \gls{machine learning} in the context of autonomous medical interventions.


==> chapters/ch4_expert_navigation/sections/2_rw.tex <==
\section{Related Work}

\paragraph{Autonomous Catheterization.} Recent advancements in \gls{machine learning} have facilitated notable progress in autonomous catheterization, particularly in foundational methodologies and early-stage implementations. Initial research efforts were directed toward supportive functionalities, including image processing and basic motion planning~\autocite{you2019automatic}. Over time, a transition toward higher levels of autonomy has been observed, with semi-autonomous navigation representing a key area of focus~\autocite{yang2017medical}. A number of studies have adopted deep \gls{reinforcement learning} approaches~\autocite{behr2019deep,karstensen2020autonomous,kweon2021deep,athiniotis2019deep,omisore2020review,omisore2021novel}, often utilizing fluoroscopic images to guide navigation and decision-making~\autocite{ji2011image}.

Despite the increasing prevalence of \gls{reinforcement learning}, alternative algorithmic strategies have also been explored. For instance, deterministic navigation along vascular centrelines has been demonstrated using the Dijkstra algorithm~\autocite{dijkstra1959note}, as applied in studies such as~\autocite{qian2019towards,cho2021image,schegg2022automated}. Other studies have employed Breadth-First Search (BFS) to enable efficient exploration of vascular structures~\autocite{fischer2022using}. While these approaches have shown promise, much of the current work remains limited to lower levels of autonomy~\autocite{yang2017medical}, often constrained by the use of physical test beds or closed-source simulation platforms.

\paragraph{Imitation Learning.} Advances in \gls{reinforcement learning} have led to the emergence of \gls{imitation learning} techniques that leverage human demonstrations for policy learning~\autocite{ho2016generative}. These techniques have proven especially valuable in complex, dynamic environments such as surgical tasks involving anatomically variable conditions. Applications of \gls{imitation learning} in robotics have included navigation in unstructured environments and precise object manipulation~\autocite{tai2018socially,finn2016guided}.

Demonstration-based methods have been widely studied in the context of endovascular navigation~\autocite{rafii2014hierarchical,rafii2013learning,assisted4,chi2018trajectory,chi2020collaborative}, with early work incorporating hidden Markov models and dynamical movement primitives~\autocite{saveriano2021dynamic}. More recent frameworks have adopted \gls{generative adversarial imitation learning} to improve generalization and policy robustness~\autocite{ho2016generative}. By leveraging insights from \gls{deep reinforcement learning}, surgical autonomy is increasingly moving toward task-level autonomy, where decision-making responsibilities are shared between human operators and robotic systems under supervised control~\autocite{dupont2021decade}.


==> chapters/ch4_expert_navigation/tables/endovascular_simulators_comparison.tex <==
\begin{table}[t]
	\scriptsize
	\caption{Endovascular simulation environments comparison.}
	\centering
	\begin{tabular}{l c c c c c}
		\toprule
		Simulator                            & Physics Engine & Catheter    & AR/VR      & Force Sensing & Open-source \\
		\midrule
		~\autocite{molinero2019haptic}       & Unity Physics  & Discretized & \xmark     & Vision-Based  & \xmark      \\
		~\autocite{karstensen2020autonomous} & SOFA           & TB theory   & \xmark     & \xmark        & \xmark      \\
		~\autocite{behr2019deep}             & SOFA           & TB theory   & \xmark     & \xmark        & \xmark      \\
		~\autocite{omisore2021novel}         & CopelliaSim    & Unknown     & \xmark     & \xmark        & \xmark      \\
		~\autocite{schegg2022automated}      & SOFA           & TB theory   & \xmark     & \xmark        & \xmark      \\
		~\autocite{you2019automatic}         & Unity Physics  & Discretized & \xmark     & Vision-Based  & \xmark      \\
		\cmidrule{1-6}
		\textbf{CathSim} (ours)              & MuJoCo         & Discretized & \checkmark & \checkmark    & \checkmark  \\
		\bottomrule
	\end{tabular}
\end{table}


==> chapters/ch4_expert_navigation/tables/force_prediction_network.tex <==
\begin{table}[h]
	\centering
	\scriptsize
	\caption{Force Prediction Network Architecture}
	\begin{tabular}{c c c c}
		\toprule
		\thead{Layer (type)} & \thead{Output Shape} & \thead{Param \#} & \thead{Nonlinearity} \\
		\midrule
		Input                & (1, 80, 80)          & 0                & -                    \\
		Conv2D               & (32, 19, 19)         & 2080             & SELU                 \\
		Conv2D               & (64, 8, 8)           & 32832            & SELU                 \\
		Conv2D               & (64, 6, 6)           & 36928            & SELU                 \\
		Flatten              & (2304)               & 0                & -                    \\
		Linear               & (768)                & 1769472          & SELU                 \\
		Linear               & (256)                & 196864           & SELU                 \\
		Linear               & (1)                  & 257              & ReLU                 \\
		\bottomrule
	\end{tabular}
	\label{ch4tab:force-network}
\end{table}


==> chapters/ch4_expert_navigation/tables/simulators_comparison.tex <==
\begin{table}[t]
	\scriptsize
	\caption{Endovascular simulation environments comparison.}
	\label{ch4tab:simulators}
	\centering
	\begin{tabular}{l c c c c c}
		\toprule
		Simulator                        & Physics Engine & Catheter    & AR/VR      & Force Sensing & Open-source \\
		\midrule
		~\cite{molinero2019haptic}       & Unity Physics  & Discretized & \xmark     & Vision-Based  & \xmark      \\
		~\cite{karstensen2020autonomous} & SOFA           & TB theory   & \xmark     & \xmark        & \xmark      \\
		~\cite{behr2019deep}             & SOFA           & TB theory   & \xmark     & \xmark        & \xmark      \\
		~\cite{omisore2021novel}         & CopelliaSim    & Unknown     & \xmark     & \xmark        & \xmark      \\
		~\cite{schegg2022automated}      & SOFA           & TB theory   & \xmark     & \xmark        & \xmark      \\
		~\cite{you2019automatic}         & Unity Physics  & Discretized & \xmark     & Vision-Based  & \xmark      \\
		\cmidrule{1-6}
		\textbf{CathSim} (ours)          & MuJoCo         & Discretized & \checkmark & \checkmark    & \checkmark  \\
		\bottomrule
	\end{tabular}
\end{table}


==> chapters/ch4_expert_navigation/tables/training_times_coparison.tex <==
\captionof{table}{Comparative training times}\label{ch4tab:training-time}
\begin{tabular}{l r r}
	\toprule
	\multirowcell{2}{\thead{Algorithm}} & \multicolumn{2}{c}{\thead{Training Time~(\(\mathbf{\unit{\hour}}\))}}                   \\
	\cmidrule{2-3}
	                                    & \thead{BCA}                                                           & \thead{LCCA}    \\
	\midrule
	Image                               & $3.00 \pm 0.11$                                                       & $2.54 \pm 0.17$ \\
	Image+Mask                          & $4.20 \pm 0.05$                                                       & $4.60 \pm 1.29$ \\
	Internal                            & $2.38 \pm 0.15$                                                       & $2.20 \pm 0.18$ \\
	Internal+Image                      & $3.15 \pm 0.28$                                                       & $3.54 \pm 0.29$ \\
	\textbf{ENN}                        & $4.61 \pm 0.22$                                                       & $4.83 \pm 0.41$ \\
	\bottomrule
\end{tabular}


==> chapters/ch4_expert_navigation/tables/user_study.tex <==
\begin{tabular}{lrr}
	\toprule
	\thead{Question}    & \thead{Average} & \thead{STD} \\
	\midrule
	Anatomical Accuracy & 4.57            & 0.53        \\
	Navigation Realism  & 3.86            & 0.69        \\
	User Satisfaction   & 4.43            & 0.53        \\
	Friction Accuracy   & 4.00            & 0.82        \\
	Interaction Realism & 3.75            & 0.96        \\
	Motion Accuracy     & 4.25            & 0.50        \\
	Visual Realism      & 3.67            & 1.15        \\
	\bottomrule
\end{tabular}









==> chapters/ch6_splineformer/sections/1_introduction.tex <==
\section{Introduction}

Cardiovascular diseases remain the leading cause of mortality globally, accounting for over one million deaths annually. Among these, coronary heart disease and cerebrovascular disease represent the most prevalent contributors~\autocite{townsend2016cardiovascular}. To address these conditions, endovascular interventions—such as \gls{percutaneous coronary intervention}, \gls{pulmonary vein isolation}, and \gls{mechanical thrombectomy}—have become essential clinical procedures~\autocite{thukkani2015endovascular,goyal2016endovascular,giacoppo2017percutaneous,lindgren2018endovascular}. These minimally invasive techniques involve the insertion and navigation of guidewires and catheters through the vascular system to reach target anatomical sites, guided by real-time intraoperative fluoroscopy. Upon reaching the destination, therapeutic actions such as thrombus removal, stent deployment, or tissue ablation are carried out to restore vascular function~\autocite{brilakis2020manual}.

Despite their efficacy, the success of these procedures is highly time-sensitive. In the case of acute ischaemic stroke, for example, delays beyond approximately $\num{7.3}$ hours significantly reduce the effectiveness of \gls{mechanical thrombectomy}~\autocite{saver2016time}. However, only a limited proportion of eligible patients receive treatment within the optimal therapeutic window, primarily due to logistical delays and procedural inefficiencies~\autocite{mcmeekin2017estimating}. These limitations underscore the need for technologies that can enhance both the speed and precision of endovascular navigation.

Fluoroscopic imaging remains central to these interventions, providing real-time visualization of the vasculature to guide instruments accurately. However, this reliance introduces several risks, including cumulative radiation exposure to patients and clinicians, and potential nephrotoxicity from contrast agents~\autocite{rudnick1995nephrotoxicity}. In addition, the manual manipulation of guidewires and catheters requires a high degree of surgical dexterity and experience, contributing to the potential for complications such as vessel perforation, distal embolization, or loss of device control~\autocite{hausegger2001complications}. These challenges point to a clear need for advanced robotic assistance and automation strategies capable of reducing operator dependency and improving procedural safety and consistency.

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{assets/system.pdf}
	\mycaption{System Overview}{The experimental setup includes three main components: \textit{i)} an anatomically accurate half-body vascular phantom model from Elastrat Sarl Ltd.; \textit{ii)} a joystick controller (robotic leader); and \textit{iii)} a robotic follower. Data are collected through teleoperation, where the robotic follower is controlled via the joystick interface.}
	\label{ch7fig:system_overview}
\end{figure}

Recent advances in \gls{machine learning} have demonstrated considerable potential to overcome many of the aforementioned limitations~\autocite{berthet2023isnake}. Among these, \gls{reinforcement learning} has emerged as a particularly promising approach for enabling precise and efficient navigation in endovascular settings. These algorithms are capable of learning complex control policies in highly dynamic and constrained environments~\autocite{chi2018trajectory,behr2019deep,kweon2021deep,cho2022sim,karstensen2022learning}. Nonetheless, the application of \gls{reinforcement learning} to real-world clinical settings remains limited, due in part to its reliance on controlled environments, specialized robotic platforms, and the absence of haptic feedback~\autocite{mofatteh2021neurosurgery,crinnion2022robotics}. Moreover, considerations related to safety, explainability, and ethical implementation remain critical as these technologies progress toward clinical deployment~\autocite{FOSCHVILLARONGA2021105528}.

In response to these challenges, a novel transformer-based model—\textbf{SplineFormer}—is introduced. This architecture is designed to exploit the geometrical structure of guidewires through the use of B-spline representations. In contrast to conventional segmentation-based methods for navigation~\autocite{abdelaziz2019toward,chi2018learning,chi2020collaborative}, SplineFormer provides an interpretable and continuous representation that is directly compatible with robotic navigation systems for endovascular procedures. The proposed approach is validated experimentally using a high-fidelity human vascular phantom and robotic setup (see Fig.~\ref{ch7fig:system_overview}), demonstrating the feasibility of autonomous guidewire navigation in a physical environment.

The main contributions of this work are summarized as follows:
\begin{itemize}
	\item A transformer-based architecture, \textbf{SplineFormer}, is proposed for learning B-spline representations of guidewire shapes, enabling smooth and geometrically constrained modelling of instrument trajectories.
	\item A training framework is designed to optimize SplineFormer for \textit{(i)} learning compact, semantically meaningful representations of guidewire shapes and \textit{(ii)} generating control actions for autonomous navigation through complex vascular anatomies.
\end{itemize}


==> chapters/ch6_splineformer/sections/2_related_works.tex <==
\section{Related Works}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\linewidth]{assets/segment_fail/AniUnet.png}\hfill
	\includegraphics[width=0.48\linewidth]{assets/segment_fail/AniSwinUnet.png}
	\mycaption{Segmentation Failure Cases}{Due to challenges in capturing thin and elongated guidewire, segmentation models often produce discontinuous segmented maps.}
	\label{ch6fig:segmentation_failure_cases}
\end{figure}


\paragraph{Guidewire and Catheter Segmentation.} Accurate modelling of guidewires and catheters is a critical challenge in endovascular interventions, as it directly impacts the precision of robotic navigation. Traditional approaches have predominantly relied on segmentation-based methods, wherein the guidewire is identified from fluoroscopic images using classical image processing techniques such as pixel intensity analysis, texture feature extraction, and histogram-based methods~\cite{brost2009_tracking,brost2010respiratory,baert2003_guidewire_tracking,wu2011learning,ma2013real}. More advanced methodologies, including the Hough transform and curvature-based techniques, have been employed to enhance detection accuracy~\cite{sheng2009automatic,kao2015_chest_CTT,bismuth2012curvilinear}. However, these approaches often exhibit limitations in the presence of low contrast, occlusions, and imaging artefacts, thereby reducing their reliability for real-time navigation in dynamic clinical environments.

Deep learning methods have introduced more robust solutions for guidewire detection and segmentation. \gls{cnn}s have been widely adopted for surgical tool localization, demonstrating significant improvements in accuracy~\cite{wang2009robust,wang2017_detection,pauly2010machine,yang2019improving,zaffino2019fully}. In particular, U-Net-based architectures~\cite{ronneberger2015u} have achieved state-of-the-art performance in segmenting guidewires from X-ray images, with refinements such as \gls{recurrent neural network}s and adaptive binarization further improving accuracy~\cite{yi2019_rnn_synthetic,ambrosini2017fully}. However, these methods primarily operate on pixel-wise segmentations, which fail to provide a structured, continuous representation of the guidewire's geometry. One common failure mode is fragmentation, where discontinuities appear in the predicted segmentation mask (Fig.~\ref{ch6fig:segmentation_failure_cases}), making it unsuitable for stable robotic navigation~\cite{zhang2022real}.

Unlike segmentation-based methods, B-spline representations offer a structured and interpretable formulation of the guidewire’s geometry. By parameterizing the guidewire as a set of control points, B-splines inherently enforce smoothness and geometric consistency, thereby reducing sensitivity to noise and enhancing navigation stability. This parametric representation is particularly advantageous for robotic applications, where compact, continuous state encodings are preferable to high-dimensional, pixel-wise outputs. Building upon this principle, the proposed approach leverages SplineFormer to directly predict B-spline parameters, enabling seamless integration into downstream robotic navigation policies.

\paragraph{Autonomous Navigation.} Autonomous navigation of guidewires within the vasculature is a highly complex task that has garnered significant attention due to its potential benefits, including reduced operative times, minimized radiation exposure, and improved procedural success rates. Recent advancements have increasingly focused on learning-based approaches to enhance the autonomous control of surgical tools, leveraging data-driven models to improve precision, adaptability, and robustness in dynamic clinical environments. \acrfull{reinforcement learning} has been extensively explored in endovascular navigation, demonstrating the capability to learn complex control policies~\cite{chi2018learning,chi2020collaborative,behr2019deep,you2019automatic,kweon2021deep,cho2022sim,karstensen2022learning}. Various \gls{reinforcement learning}-based approaches have been proposed to train agents for autonomous guidewire navigation. However, their performance is highly contingent on the quality of the state representation. Many existing methods rely on raw image-based observations, which are inherently high-dimensional and lack an explicit geometric structure, posing challenges for interpretability and efficient decision-making.

To mitigate these challenges, several studies have integrated \gls{learning from demonstration} techniques, such as \gls{generative adversarial imitation learning}~\cite{chi2020collaborative} and \gls{behavioural cloning}~\cite{chi2018learning}, where expert trajectories serve as supervisory signals to guide learning. These approaches have demonstrated potential in reducing the sample complexity of \gls{reinforcement learning} algorithms by incorporating expert knowledge. However, existing methods often suffer from poor generalization due to the absence of structured state representations. In contrast, the proposed approach employs B-spline representations to construct a compact and structured state space, facilitating more stable and interpretable endovascular navigation.


==> chapters/ch6_splineformer/sections/3_method.tex <==
\section{B-Spline Representation for Autonomous Endovascular Navigation}

Accurate geometric modelling of curvilinear guidewires and catheters is essential for precise navigation and control in interventional procedures. Conventional approaches primarily rely on dense image-based representations~\cite{wu2014fast}, which capture the tool’s shape at the pixel level but lack an intrinsic parametric structure suitable for real-time navigation. To overcome these limitations, SplineFormer (Fig.~\ref{ch6fig:main_architecture}) is developed, adopting a B-spline-based representation to encode the guidewire’s shape in a compact, continuous, and structured form. By directly parameterizing the guidewire’s geometry, this approach eliminates the need for post-processing steps required by segmentation-based methods, facilitating seamless integration into downstream robotic navigation policies.




\subsection{B-Spline Representation for Guidewire Modelling}

\begin{figure}[h]
	\centering
	\includegraphics[width=.8\linewidth]{figures/bspline.jpg}
	\mycaption{B-Spline Guidewire Representation}{A guidewire can be represented as a continuous B-spline curve.}\label{ch6fig:bspline-representation}
\end{figure}

A B-spline curve represents the guidewire’s shape using a set of control points and a non-decreasing sequence of knots, providing a smooth and flexible parametric formulation (Fig.~\ref{ch6fig:bspline-representation}). This structured encoding inherently enforces continuity and geometric consistency, enabling stable and anatomically realistic trajectory adjustments during navigation. A B-spline curve \( \mathbf{C}(t) \) of degree \( p \) is defined as:

\begin{equation}
	\mathbf{C}(t) = \sum_{i=0}^{n} \mathbf{P}_i B_{i,p}(t),
\end{equation}
where \( \mathbf{P}_i \) denotes the control points, and \( B_{i,p}(t) \) represents the B-spline basis functions of degree \( p \), defined over the knot vector \( t_0, t_1, \dots, t_m \). The basis functions \( B_{i,p}(t) \) are computed recursively as follows:

\begin{equation}
	B_{i,0}(t) =
	\begin{cases}
		1, & \text{if } t_i \leq t < t_{i+1}, \\
		0, & \text{otherwise}.
	\end{cases}
\end{equation}

\begin{equation}
	B_{i,p}(t) = \frac{t - t_i}{t_{i+p} - t_i} B_{i,p-1}(t) + \frac{t_{i+p+1} - t}{t_{i+p+1} - t_{i+1}} B_{i+1,p-1}(t)
\end{equation}

Additionally, the constraint $\sum_{i=0}^{m-p-1} B_{i,p}(t) = 1$
ensures that the guidewire’s shape remains consistent across varying imaging conditions, enabling real-time inference. To balance smoothness and computational efficiency, the B-spline degree is set to \( p=3 \). The number of control points \( n \) is dynamically selected based on the guidewire’s length, optimizing flexibility while maintaining model stability. The knot vector follows a uniform non-decreasing sequence, ensuring numerical robustness during optimization.

\begin{figure}[ht]
	\centering
	\includegraphics[width=\linewidth]{figures/main_architecture.drawio.png}
	\mycaption{SplineFormer Network Architecture}{The input fluoroscopic image \( X \) is processed by a visual transformer encoder that divides the image into patches, embeds them, and generates visual feature representations \( X' \). Simultaneously, a positional encoder processes embeddings of the target sequence. These encoded features are fed into a transformer decoder composed of \( N_D \) layers. Using masked self-attention and cross-attention mechanisms, the decoder sequentially generates the B-spline control points \( \mathbf{P}_i \) and knots \( t_i \) that define the guidewire's geometry. The decoder predicts these parameters by projecting its outputs onto the B-spline dimensionality, yielding pairs \( \{\mathbf{P}_0, t_0\}, \{\mathbf{P}_1, t_1\}, \dots, \{\mathbf{P}_n, t_n\} \), which are subsequently passed to a multi-layer perceptron (MLP) to predict the navigation action \( \mathbf{a}_t = (\Delta x, \theta) \). An independent tip predictor module initializes the generation by predicting the starting point \( \{\mathbf{P}_0,t_0\} \).}
	\label{ch6fig:main_architecture}
\end{figure}




\subsection{SplineFormer Network Architecture}

SplineFormer (Fig.~\ref{ch6fig:main_architecture}) is built upon a \gls{vit} backbone~\cite{dosovitskiy2020image} with \( N_e = 12 \) encoder layers and \( N_D = 6 \) decoder layers. Each encoder layer employs \( H = 8 \) attention heads with a hidden dimension of \( d_k = 512 \). Input fluoroscopic images are resized to \( 224 \times 224 \) pixels and tokenized into \( 16 \times 16 \) patches. The model is trained using the Adam optimizer on an NVIDIA A100 GPU with a batch size of 32, reaching convergence after 120K iterations.


\paragraph{Encoder.} Two encoders are employed to extract structured features from fluoroscopic images, enabling precise guidewire representation for downstream navigation. The first encoder follows a \gls{vit}, where the input image \(X \in \mathbb{R}^{H \times W}\) is divided into \(N_P\) patches, computed as:

\begin{equation}
	N_P = \frac{H}{|P|} \times \frac{W}{|P|},
\end{equation}
where \(|P|\) denotes the patch size. These patches are flattened into a 1D tensor and embedded into a latent feature space via a linear projection layer. The second encoder is a sinusoidal positional encoder~\cite{vaswani2017attention}, applied to both the image patches \( P \) and the target sequence \( Y_{\text{TGT}} \in \mathbb{R}^{S \times E} \), where \( S \) and \( E \) denote the sequence length and embedding dimension, respectively. This dual encoding mechanism ensures that the extracted features capture both local and global information, essential for accurately predicting the guidewire's shape.

The transformer encoder consists of \(N_e\) stacked identical layers, each comprising a \gls{multi-head self-attention} module followed by a positional \gls{feed forward network}. The \gls{multi-head self-attention} module contains \(H\) parallel attention heads, each computing a scaled dot-product attention function. This architecture enables the network to attend to both local and global contextual information, which is critical for capturing the intricate bending and twisting of the guidewire during navigation. The outputs from all heads are aggregated via a learnable linear transformation \( W^O \), formulated as:

\begin{equation}
	\operatorname{MHA}(Q,K,V) = \operatorname{Concat}(h_1, h_2, \dots, h_H)W^O,
\end{equation}
where the scaled dot-product attention for each head is computed as:

\begin{equation}
	\operatorname{Attention}(Q,K,V) = \operatorname{Softmax} \left(\frac{QK^T}{\sqrt{d_k}}\right) V,
\end{equation}
where \( \{Q,K,V\} \in \mathbb{R}^{N_q \times d_k} \) represent the query, key, and value matrices, respectively.

Following the \gls{multi-head self-attention} module, the positional \gls{feed forward network} is implemented using two fully connected layers with GELU activation and dropout regularization:

\begin{equation}
	\operatorname{FFN}(x) = \operatorname{FC_2} \left( \operatorname{Dropout} \left( \operatorname{GELU} \left( \operatorname{FC_1}(x) \right) \right) \right)
\end{equation}

To enhance stability, each sublayer is equipped with a residual connection, followed by layer normalization:

\begin{equation}
	x^{\text{out}}= \operatorname{LayerNorm} \left( x^{\text{in}} + \operatorname{Sublayer}(x^{\text{in}}) \right)
\end{equation}


\paragraph{Decoder.} The decoder consists of \(N_D\) transformer layers that sequentially generate the B-spline control points and corresponding knots, defining the guidewire’s smooth representation. Each layer comprises masked self-attention, multi-head cross-attention, and a \gls{feed forward network}~\cite{vaswani2017attention}. This hierarchical structure enables the model to iteratively refine the predicted guidewire shape while capturing its curvature and spatial relationships in a compact form. The decoder’s final output is projected onto the B-spline parameter space, yielding the structured representation:

\begin{equation}\label{eq:splineformer-output}
	\{ \mathbf{P}_0, t_0 \}, \{ \mathbf{P}_1, t_1 \}, \dots, \{ \mathbf{P}_n, t_n \},
\end{equation}
where \( \mathbf{P}_i \) are the control points and \( t_i \) are the associated knot values. This formulation defines the guidewire’s geometry as a continuous parametric curve \( \mathbf{C}(t) \), enabling accurate and interpretable navigation. By leveraging a structured and smooth state representation, this approach ensures both robust real-time inference and geometrically consistent trajectory estimation.


\paragraph{Tip Predictor.} The tip predictor module establishes a geometrically consistent anchor for guidewire shape prediction by estimating the initial tip position in the image. It consists of a series of convolutional layers with \gls{relu} activations, followed by linear transformations that regress the tip coordinates. Given an input image \( I \), the module predicts the tip location:

\begin{equation}
	\mathbf{P}_0 = (x_0, y_0),
\end{equation}
which serves as the initial token for autoregressive guidewire prediction, ensuring that the generated trajectory remains spatially coherent and well-anchored.

The encoder and tip predictor interact in a complementary manner: the encoder extracts hierarchical guidewire features from the fluoroscopic image, while the tip predictor directly predicts the initial tip position from these encoder derived feature representations. By leveraging the multiscale contextual information captured by the encoder, such as vessel boundaries, local intensity patterns, and structural cues, the tip predictor gains a richer understanding of vessel topology, allowing it to produce a more precise and anatomically valid starting point. This is crucial, as an inaccurate tip estimation could introduce propagation errors in the subsequent trajectory prediction. The estimated tip $\mathbf{P}_0$ is then passed to the decoder, which generates the full guidewire trajectory based on this initialization.




\subsection{Loss Function}

The shape loss function \( \mathcal{L}_{\rm shape} \) combines three weighted components, each scaled by a corresponding hyperparameter \( \lambda \):
\textit{(i)} A \gls{mean squared error} loss applied to the predicted and target sequences of control points and knots.
\textit{(ii)} A \gls{binary cross-entropy} loss for the End-of-Sequence (EOS) prediction.
\textit{(iii)} A curvature consistency loss, computed by sampling the predicted B-spline curve at \(n\) parameter values \(t_k\), uniformly distributed over the valid parameter range \( [t_p, t_{m-p}] \).

The sampled parameter values are defined as:

\begin{equation}
	t_k = t_p + \frac{k}{n-1} (t_{m-p} - t_p), \quad k = 0, 1, \dots, n-1
\end{equation}

The complete loss function is:

\begin{equation}
	\begin{split}
		\mathcal{L}_{\text{shape}} = \frac{1}{N} \sum_{i=1}^N \bigg(
		 & \lambda_a \big(\|t_i - \hat{t}_i\|^2 + \|\mathbf{P}_i - \hat{\mathbf{P}}_i\|^2\big) +                            \\
		 & \lambda_b \big( -\mathbf{s}_i \log(\hat{\mathbf{s}}_i) - (1 - \mathbf{s}_i) \log(1 - \hat{\mathbf{s}}_i) \big) + \\
		 & \lambda_c \left\| \mathbf{C}(t_k) - \mathbf{\hat{C}}(t_k) \right\|^2 \bigg)
	\end{split}
\end{equation}

The output of SplineFormer is a predicted sequence of control points and knots. This sequence serves not only as a shape descriptor but also as the input state for downstream action prediction. By coupling shape inference directly to action generation, the model forms a single cohesive pipeline from image to navigation decision.




\subsection{Policy Training}

The predicted control points and knots from Eq.~\ref{eq:splineformer-output} are directly passed to a \gls{mlp} that predicts the next navigation action. The \gls{mlp} processes these inputs—along with derived curvature features—through fully connected layers with \gls{relu} activations, producing:

\begin{equation}
	\mathbf{a}_t = (\Delta x, \theta),
\end{equation}
where \( \Delta x \) denotes the translation step and \( \theta \) denotes the rotation angle. This policy network is trained by minimizing the mean squared error between predicted and expert actions:

\begin{equation}\label{ch6eq:spline_loss}
	\mathcal{L}_{\text{action}} = \sum_t \|\mathbf{a}_t - \mathbf{a}_t^*\|^2
\end{equation}

This direct dependence between the predicted guidewire shape and the navigation action ensures that every control decision is grounded in the current estimate of the guidewire’s geometry, providing both physical consistency and a structured link between perception and control.


==> chapters/ch6_splineformer/sections/5_conclusions.tex <==
\subsection{Discussion}

SplineFormer is presented as a new transformer network for predicting continuous guidewire geometries using a B-spline representation, enabling efficient encoding for real-time navigation. By parameterizing the guidewire with control points and knots, this approach ensures geometric consistency and provides a compact state representation for downstream robotic control. However, small variations in B-spline parameters can introduce spatial misalignment, affecting trajectory accuracy. In robotic experiments, SplineFormer successfully cannulated the \gls{bca} but failed in the \gls{lcca}, consistent with prior findings~\cite{chi2020collaborative,jianu2024cathsim}. The \gls{lcca}'s sharper turns, narrower lumen, and abrupt bifurcation angle increase resistance and the risk of collision, challenging model generalization. These findings highlight the need for improved adaptability in high-curvature vascular structures.

\subsection{Limitations}

While SplineFormer provides a structured and interpretable representation for autonomous navigation, its reliance on B-spline parameterization makes it sensitive to perturbations, which can affect trajectory stability. Additionally, its failure in \gls{lcca} navigation reinforces the well-documented challenges of traversing high-curvature vascular regions~\cite{chi2020collaborative}. The \gls{lcca}'s complex morphology makes navigation inherently more difficult than in the \gls{bca}, limiting policy generalization. Addressing these challenges will require adaptive trajectory optimization, uncertainty-aware planning, and biomechanical modelling to improve robustness. Despite these constraints, SplineFormer demonstrates the viability of shape-driven navigation strategies, motivating further research into learning-based autonomous interventions.

The contributions of SplineFormer represent a significant advancement in geometric modelling for endovascular navigation, offering a novel approach that complements the earlier components of this thesis. While CathSim provided the simulation environment, the Expert Navigation Network demonstrated multimodal learning capabilities, and Guide3D addressed data scarcity, SplineFormer introduces an innovative geometric representation that directly enhances navigation accuracy and interpretability. Together, these integrated contributions establish a comprehensive framework that addresses multiple facets of the autonomous endovascular navigation challenge, from simulation and data availability to perception and control.

\section{Conclusions}

SplineFormer is introduced as a spline-based framework for autonomous endovascular navigation that encodes guidewire geometry in a compact and structured latent representation. The method enhances trajectory planning and real-time decision-making, providing a foundation for precision-driven robotic control. While SplineFormer performs well in structured environments, addressing its limitations in high-curvature navigation is essential for real-world deployment. Future work will focus on adaptive learning strategies, biomechanical modelling, and preclinical validation to enhance generalization. By leveraging explainable curvilinear representations, SplineFormer shows the potential for fully autonomous endovascular interventions, contributing to safer and more efficient vascular navigation.


==> chapters/ch6_splineformer/tables/bc_metrics.tex <==
\begin{table}[h]
	\caption{Navigation Results}\label{ch7tab:navigation-result}
	\begin{center}
		\begin{tabular}{c c c}
			\toprule
			             & \thead{BCA}                & \thead{LCCA}              \\
			\midrule
			Success Rate & \(50\%\)                   & -                         \\
			Time         & \(2.5 \pm 0.76\text{min}\) & \(3.0 \pm 0.0\text{min}\) \\
			\bottomrule
		\end{tabular}
	\end{center}
	\vskip -0.1in
\end{table}


==> chapters/ch6_splineformer/tables/image_pred_metrics.tex <==
\begin{table}[ht]
    \caption{My caption}\label{splineformer-tab:segment}
\begin{center}
\begin{tabular}{c c c c c c}
\toprule
    & Dice & fsim & lpips & pixel acc & jaccard   \\
\midrule
UNet    & 0.999 & 0.9899 & & & \\
Swin-UNet & 0.358 & 0.985 & 0.055 & 0.991 & \\
% SwinUNet  &   & 0.000 & 0.0431 & &  \\
SplineFormer & 0.066 & 0.963 & 0.0368 & 0.995 & 0.035\\

\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table}


       %    dice             0.001492705661803484
       %    fsim               0.999291181564331
       %    lpips                     0.0
       %  pixel_acc           0.9856394529342651
       %  precision          0.0007466510869562626
       %   recall             0.9994094967842102
       % specificity          0.9856393337249756
       
% SWIN UNET
%          dice              0.35810133814811707
%          fsim              0.9849305152893066
%         jaccard                    0.0
%          lpips             0.05450419709086418
%        pixel_acc           0.9909709692001343
%        precision           0.22002705931663513
%         recall             0.9985209107398987
%       specificity          0.9909501671791077


% \begin{table}[ht]
% \caption{My caption}
% \begin{center}
% \begin{tabular}{c c c}
% \toprule
%     & UNet & SplineForme \\
% \midrule
%     SSIM  & 0.999 & 0.9899 \\
%     LPIPS & 0.000 & 0.0431 \\
% \bottomrule
% \end{tabular}
% \end{center}
% \vskip -0.1in
% \end{table}


==> chapters/ch6_splineformer/tables/navigation.tex <==
\begin{table*}[t]
	\begin{minipage}[b]{0.7\linewidth}
		\centering
		\resizebox{\linewidth}{!}{
			\setlength{\tabcolsep}{0.2 em} % for the horizontal padding
			{\renewcommand{\arraystretch}{1.8}% for the vertical padding
				\begin{tabular}{c|c|c|cc|cc}
					\hline
					\multirow{2}{*}{\textbf{Method}}                                                                     & \multirow{2}{*}{\textbf{Setup}}                          & \multirow{2}{*}{\textbf{Explainable?}} & \multicolumn{2}{c|}{\textbf{BCA}}          & \multicolumn{2}{c}{\textbf{LCCA}}                                                                  \\ \cline{4-7}
					                                                                                                     &                                                          &                                        & \multicolumn{1}{c|}{\textit{Success (\%)}} & \textit{Time (\text{s})}          & \multicolumn{1}{c|}{\textit{Success (\%)}} & \textit{Time (s)} \\ \hline
					\begin{tabular}[c]{@{}c@{}}Expert  Teleoperation\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}Fully Manual\end{tabular}     & \_                                     & \multicolumn{1}{c|}{100}                   & \(32.1\pm9.1\)                    & \multicolumn{1}{c|}{100}                   & \(25.0 \pm 6.7\)  \\ \hline \hline
					\begin{tabular}[c]{@{}c@{}}GAIL-PPO\cite{chi2020collaborative}\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}Semi-Autonomous\end{tabular}  & No                                     & \multicolumn{1}{c|}{69.4}                  & \(52.1\pm9.9\)                    & \multicolumn{1}{c|}{72.2}                  & \(76.5\pm24.1\)   \\ \hline
					\hline
					\begin{tabular}[c]{@{}c@{}}Behavior Cloning~\cite{chi2020collaborative}\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}Fully Autonomous\end{tabular} & No                                     & \multicolumn{1}{c|}{5.60}                  & \(>200\)                          & \multicolumn{1}{c|}{\_}                    & -                 \\ \hline
					\rowcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{SplineFormer} \textbf{(ours)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Fully Autonomous\end{tabular} & Yes                                    & \multicolumn{1}{c|}{50.0}                  & \(150 \pm 45.6\)                  & \multicolumn{1}{c|}{\_}                    & -                 \\ \hline
				\end{tabular}
			}}
		\vspace{5ex}
		\caption{Endovascular navigation results.
			% \vspace{5ex}
		}
		\label{tab:NavResult}
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=0.8\textwidth,height=0.9\linewidth]{assets/setup.pdf}
		\vspace{2 ex}
		\captionof{figure}{Navigation setup.}
		%\vspace{-1ex}
		\label{fig:target-setup}

	\end{minipage}
\end{table*}


==> chapters/ch6_splineformer/tables/shape_comparison.tex <==
\begin{table}[ht]
  \caption{My caption}\label{splineformer-tab:shape-comparison}
\begin{center}
\begin{tabular}{c c c c}
\toprule
   & METE & MERS & MAXEd \\
\midrule
  Time  & \(2.50 \pm	0.76\) min & b & \\
  Success Rate & \(50\%\) & d &a\\
\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table}


==> postamble/appendices/cathsim/main.tex <==
\section{CathSim}

\subsection{CathSim Design Details}

\textbf{Aortic Models.} In addition to Type-I Aortic Arch model which is mainly used in our experiments, we incorporate three distinct aortic models to enrich our anatomical dataset. These models include a high-fidelity Type-II aortic arch and a Type-I aortic arch with an aneurysm, both sourced from Elastrat, Switzerland. Furthermore, a low tortuosity aorta model, based on a patient-specific CT scan, is included. With these three additional representations, our simulator contains four distinct aorta models. These models aim to enhance the diversity and accuracy of aortic structures available for research and educational endeavors. These aortas are visualized in Fig.~\ref{fig:three aorta}.

\begin{figure}[ht]
	\centering
	\subfloat[Type-I (Aneurysm)]{\includegraphics[width=0.3\textwidth]{assets/aneurysm.png}}
	\hfill
	\subfloat[Type-II]{\includegraphics[width=0.3\textwidth]{assets/type2.png}}
	\hfill
	\subfloat[Low Tortuosity]{\includegraphics[width=0.3\textwidth]{assets/low_tort.png}}
	\caption{Aortic Models.}
	\label{fig:three aorta}
\end{figure}


\subsection{CathSim Speed Evaluation}

\begin{sidebysidefigures}[.5]
	\begin{leftfigure}
		\adjustimage{left}{assets/episode_time.png}
		\captionof{figure}{CathSim training speed.}
		\label{app1fig:fps}
	\end{leftfigure}%
	\begin{rightfigure}
		\vspace{0.35cm}
		\input{tables/training_times_coparison.tex}
	\end{rightfigure}

\end{sidebysidefigures}


\paragraph{Training Speed.} As illustrated in Fig.~\ref{app1fig:fps}, we provide a comparison of frames per second (FPS) for the various algorithms we employed during model training. It is evident that utilizing solely the internal state space, comprised of joint positions and velocities, facilitates expedited training processes. In contrast, integrating all modalities into the training process results in its deceleration. The most significant computational demand arises from the dual convolutional neural networks utilized in both the image and mask representations. However, despite this load, the algorithms exhibit respectable computational speed, even during the training phase. Our simulator supports approximately $40$ to $80$ frames per second performance for all implemented algorithms, underscoring the computational speed of our simulation environment. Moreover, we provide the training times in terms of hours for the different modalities in Table~\ref{app1tab:training-time}.

% \section{Expert Navigation Network Implementation}
% \label{app_expert_nav}

% \textbf{Observation Space.} We incorporated a range of observations to provide the agent with an extensive understanding of the environment. A grayscale image of dimensions $80 \times 80$ (denoted by \(I \in [0, 1]^{80 \times 80}\)) is generated as a visual clue, which is accompanied by the ground truth binary segmentation mask \(S \in \{0,1\}^{80 \times 80}\). The mask \(S[i,j] = 1\) is validated only when the pixel coordinates \((i,j)\) are part of set \(A\), the pixels that constitute the guidewire. Furthermore, to enhance the reinforcement learning problem's optimization, we also included the ground truth joint positions \(Q \in \mathbb{R}^{168}\) and joint velocities \(V \in \mathbb{R}^{168}\). These joint values provide detailed mechanical insight into the guidewire's state, enriching the agent's knowledge base and facilitating informed decision-making.

% \textbf{Action Representation.} In CathSim, the essential actions are denoted by translation \(a_t \in [-1,1]\) and rotation $a_r \in [-1,1]$. At each time step, the agent generates these actions, which are collectively represented by the vector $a \in [-1,1]^2$. Here, a positive $a_t$ denotes forward movement, while a negative $a_t$ signifies a backward movement. Similarly, a positive $a_r$ corresponds to a clockwise guidewire rotation, while a negative $a_r$ indicates an anticlockwise rotation. The selection of translation and rotation actions in CathSim closely mirrors the actions in real-world endovascular procedures, as described by~\autocitet{kundrat2021mr}. By faithfully reproducing the motions of an actual robot, the simulation environment better replicates real-world situations. This enables the reinforcement learning agent to acquire policies that can be feasibly implemented in a physical robot, thereby augmenting the practical value and applicability of the behaviors learned.

% \textbf{Reward Function.} Our employed reward system is dense, and it hinges on the spatial position of the guidewire tip in relation to the goal. Formally, the reward $r$ is determined by the function $r(p_t, g)=-d(p_t,g)$, where $d(p_t,g)=||p_t-g||$ characterizes the distance between the position $p$ of the guidewire tip at time $t$ and the target $g$. If the guidewire tip lies within a distance threshold $\delta$ of the target $g$, the agent is conferred a positive reward $r$. For our research, we adopted a $\delta$ of $4\unit{\milli\metre}$ and assigned a task completion reward of $r=10$. Consequently, we end up with the following reward function:

% \begin{equation}
% r(h_t, g) = 
%     \begin{cases}
%     10 & \text{if} \quad d(h,g) \leq \delta \\
%     -d(h,g) & \text{otherwise} 
%     \end{cases}
% \end{equation}

% \textbf{Training Details.} The experiments were conducted on an  NVIDIA RTX 2060 GPU (\(33\unit{\mega\hertz}\)) system on an Ubuntu 22.04 LTS based operating system. Furthermore, the system contained an AMD Ryzen 7 5800X 8-Core Processor with a total of 16 threads with \(64\unit{\giga\byte}\) of RAM. All experiments used PyTorch, whilst for the Soft Actor Critic implementation we used stable baselines~\autocite{stable-baselines3}. The training was carried out for a total of $600,000$ time steps using a total of $5$ different random seeds, resulting in a training time bounded between $2$ and $5$~hours. Each episode has two terminal states, one which is time-bound (i.e., termination of an episode upon reaching a number of steps) and one which is goal bound (i.e., the agent achieves the goal $g$).



% \begin{minipage}[t]{\textwidth}
%     % \vspace{-1cm}
%     \begin{minipage}[t][][b]{0.6\textwidth}
%         \centering
%         \scriptsize
%         \input{tables/ENN_architecture}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t][][b]{0.35\textwidth}
%         \begin{minipage}[t]{\textwidth}
%             \scriptsize
%             \centering
%             \input{tables/ENN_hyperparams}

%         \end{minipage}
%     \end{minipage}
% \end{minipage}

% \textbf{Networks.} We employ multiple feature extractors to dissociate the dominant features within our Expert Navigation Network~(ENN). Specifically, we use a convolutional neural network (CNN~\autocite{mnih2015human}) to extract the image-based features, resulting in two latent features $J_I$ and $J_S$ that represent the top camera view and guidewire segmentation map. The CNN is composed of $3$ convolutional layers with a $\operatorname{ReLU}$~\autocite{agarap2018deep} activation function, followed by a flattening operation. We also concatenate joint positions~$Q$ and joint velocities~$V$ to generate a joint feature vector $J_J=Q \parallel P$ of dimensionality $336$ which is then passed through the MLP. These features are concatenated to form a single feature vector $J=J_I \parallel J_S \parallel J_J$, which is fed into a policy network $\pi (a_t,\theta)$. Both network architectures are presented in Table~\ref{tab:network-architectures-cnn-mlp}.

% \textbf{SAC.} Our primary reinforcement learning method is the soft actor-critic~(SAC)~\autocite{haarnoja2018soft}. Soft actor-critic (SAC) is a model-free reinforcement learning algorithm that learns a stochastic policy and a value function simultaneously. The objective function of SAC combines the expected return of the policy and the entropy of the policy, which encourages exploration and prevents premature convergence to suboptimal policies. The algorithm consists of three networks, namely a state-value function $V$ parameterized by $\psi$, a soft $Q$-function $Q$ parameterized by $\theta$, and a policy $\pi$ parameterized by $\phi$. The parameters we employ are present in Table~\ref{tab:sac}. For the policy network, we use a composition of linear layers to handle and transform the input data.



% \section{Downstream Tasks}
% \label{app_downstream_task}

% \subsection{Imitation Learning}


% \textbf{Network.} The architecture of our network for the Behavioral Cloning (BC) algorithm consists of a sequence of specialized layers that gradually transform the input data. The process initiates with the input, formatted as a tensor of dimensions (1, 80, 80), which is passed through three Conv2D layers. All of these layers employ the Rectified Linear Unit (ReLU) as their activation function. Upon passing through the Conv2D layers, the output tensor is reshaped into a single dimension by a flattening layer, facilitating the shift from convolutional to linear layers. The flattened output is then processed by a Linear layer utilizing the ReLU activation function. Finally, an additional Linear layer, without an activation function, delivers the final output of the network. This last layer provides raw scores, which are interpreted directly as the network's output, mirroring the decisions made by the BC algorithm. The network architecture is illustrated in Table~\ref{tab:bc-network}.


% \begin{minipage}[t]{\textwidth}
%     \begin{minipage}[t][][b]{0.6\textwidth}
%         \centering
%         \scriptsize
%         \centering
%         \scriptsize
%         \input{tables/BC_architecture}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t][][b]{0.35\textwidth}
%         \begin{minipage}[t]{\textwidth}
%             \scriptsize
%             \centering
%             \input{tables/BC_hyperparams}
%         \end{minipage}
%     \end{minipage}
% \end{minipage}

% \begin{table}[h]

% \end{table}

% \textbf{Training.} To train the BC algorithm, we employ a set of hyperparameters, as listed in Table~\ref{tab:bc-hyperparameters}. The training procedure makes use of a batch size of \(32\). The Adam~\autocite{kingma2014adam} optimizer is utilized to minimize the loss function. We set the learning rate and entropy coefficient to \(1 \times 10^{-3}\), controlling the step size at each iteration of the optimization and regularizing the policy towards a more exploratory behavior, respectively. The training process spans over \(800\) epochs, each epoch consisting of a complete pass through the entire dataset, providing the model ample opportunity to converge to an optimal solution.




% \subsection{Force Prediction}

% \input{tables/force_prediction_network}

% \textbf{Network.} We utilize a hybrid architecture comprising a CNN followed by an MLP, with a grayscale image as the input. The network architecture includes three Conv2D layers that apply convolution operations to the input tensor. Each of these convolutional layers employs the Scaled Exponential Linear Unit (SELU~\autocite{klambauer2017selfnormalizing}) as the activation function, encouraging self-normalization and improving the network's capability to propagate gradients deeply into the architecture. Subsequent to the Conv2D layers, a flattening layer reshapes the output into a one-dimensional tensor. Thereafter, the architecture implements three Linear layers. The initial two layers use the SELU activation function, while the final one adopts the Rectified Linear Unit (ReLU~\autocite{agarap2018deep}) activation function. This amalgamation of multiple linear layers, each paired with a distinct non-linear activation function, enables the network to learn complex patterns in the input data, leading to the network's final output. Table~\ref{tab:force-network} shows the force prediction network architecture.

% \textbf{Training.} We employed the NAdam optimizer~\autocite{dozat2016incorporating} to train our model, setting the initial learning rate at \(4\times10^{-4}\). This was coupled with a SELU activation function to enhance self-normalization and facilitate gradient propagation. To dynamically adjust the learning rate during the training process, we used a OneCycle learning rate scheduler~\autocite{smith2018superconvergence}, and the training was conducted for a total of \(30\) epochs.

% \textbf{Data Management.} In terms of data management, we divided the original dataset into training, testing, and validation subsets according to the total time steps. Initially, we allocated \(20\%\) of the total time steps to the test set. Subsequently, the remaining data was partitioned into a validation set and training set, with the validation set representing \(20\%\) of the leftover steps. This procedure was followed for each experimental run of our force prediction model, generating corresponding sets of transitions. Of particular note, the test set consistently stemmed from our largest trajectory dataset—the \(100K\) dataset. For each training run, we designated \(20\%\) of this dataset for validation, utilizing the remaining portion for training. The model's performance was assessed using the originally separated test set. By adhering to this structured and consistent methodology, we ensured a rigorous and equitable evaluation of our model's performance across multiple runs.




% Shape prediction, especially for guidewires, is instrumental in reducing vasculature stress and optimizing control performance. This ultimately results in a substantial reduction in complication risks~\autocite{shi2016shape}. Efforts to attain precise shape prediction have led to significant investments in shape-sensing technologies. One noteworthy example is the FBG-sensors~\autocite{chitalia2020towards}, tailored for shape approximation. However, the incorporation of these sensors presents several challenges. They not only entail material costs and augment the instrument size but also limit navigational abilities and necessitate major alterations to optimize guidewire features, including stiffness. To navigate these environments, alternatives have been sought, including reconstructions from bi-planar scanner images or those anchored in precise kinematics~\autocite{shi2016shape}. While deep learning emerges as a promising solution, especially in terms of cost mitigation, it inherently demands extensive data.

% \begin{figure}[h]
%     \centering
%     \subfigure{\includegraphics{assets/rebuttal/shape_prediction.png}}
%     \caption{Shape Prediction}
%     \label{fig:shape}
% \end{figure}

% We posit that our simulator can be instrumental in furnishing the necessary data to train models that use images to approximate instrument shapes. To affirm this, we have juxtaposed image observations of shape $80\times80$ with the real 3D positions of the guidewire bodies $p$, facilitating the guidewire shape reconstruction from 2D images. Using this data, we trained a CNN, leveraging the NAdam optimizer~\autocite{dozat2016incorporating} and a refined loss function encompassing the Huber Loss~\autocite{huber1992robust} with a $\delta=1$:

% \begin{equation}
% \mathcal{L}_{\text{Huber}}(y, \hat{y}) = \begin{cases} 
%                                     \frac{1}{2}(y - \hat{y})^{2} & \text{if } \left | y - \hat{y} \right | < \delta \\
%                                     \delta \left( \left| y - \hat{y} \right| - \frac{\delta}{2} \right) & \text{, otherwise}
%                                 \end{cases}\,,
% \end{equation}

% Here, $y$ denotes the ground truth positions of the guidewire bodies, and $\hat{y}$ signifies the predicted positions. A regularization term, $\mathcal{L}_{\text{reg}}$, is introduced to ensure the guidewire's geometric structure remains intact, assuming an interbody distance of $2\unit{mm}$:

% \begin{equation}
%     \mathcal{L}_{\text{reg}} = \frac{1}{n-1} \sum_{i=1}^{n-1} \left| \lVert \hat{y}_{i+1} - \hat{y}_i \rVert_2 - 0.002 \right|
% \end{equation}

% The combined loss is then represented as:

% \begin{equation}
%     \mathcal{L}= \alpha \mathcal{L}_{\text{Huber}}(y, \hat{y}) + \beta \mathcal{L}_{\text{reg}}\,,
% \end{equation}

% Our comparative analysis between the actual guidewire shape and its prediction is visually represented in Fig.~\ref{fig:shape}. The close approximation of the guidewire shape from the 2D image underscores our simulator's potential. 

% Such findings highlight the capacity of our simulator to enhance auxiliary tasks, enabling researchers to utilize the simulator for data-driven model samples. While this provides a foundation, a deeper delve into simulation to real transfer nuances is warranted in future research. Nevertheless, considering the exorbitant costs of real-world data acquisition, our simulator stands out as a pivotal tool in the evolution of these methodologies.


==> postamble/appendices/code/cathsim/code_listing.tex <==
\begin{longlisting}
	\mycaption{Example Source Code - Add Two Integers}{Python code to perform addition of two integers.}
	\label{lst:add_two_integers} \inputminted[firstline=1]{python}{quickstart.py}
\end{longlisting}

\clearpage


==> postamble/appendices/code/cathsim/main.tex <==
\subsection{CathSim}

This appendix reproduces the full README for \emph{CathSim: An Open-source Simulator for Endovascular Intervention}. For more details, please refer to the project page at \url{https://airvlab.github.io/cathsim/} and the paper at \url{https://arxiv.org/abs/2208.01455}.


\subsubsection{Requirements}

\begin{itemize}
	\item Ubuntu (tested with Ubuntu 22.04 LTS)
	\item Miniconda (tested with Miniconda 23.5)
	\item Python 3.9
\end{itemize}

If \texttt{miniconda} is not installed, run the following script (assuming \texttt{bash} is your shell):

\begin{longlisting}
	\mycaption{Miniconda Installation}{How to install Miniconda.}
	\inputminted[firstline=1]{bash}{postamble/appendices/code/cathsim/code/miniconda_install.sh}
\end{longlisting}

\subsubsection{Installation}

First, create a conda environment and install the package:


\begin{longlisting}
	\mycaption{Create Conda Env}{How to create a conda env.}
	\inputminted{bash}{postamble/appendices/code/cathsim/code/create_env.sh}
\end{longlisting}

\subsubsection{Quickstart}

You can quickly set up a Gym-compatible environment using the \texttt{make\_dm\_env} function along with the \texttt{DMEnvToGymWrapper}. For example:

\begin{longlisting}
	\mycaption{CathSim as Gym Env}{Demonstration of how CathSim can be used as a Gym environment.}
	\inputminted[firstline=1]{python}{postamble/appendices/code/cathsim/code/cathsim_gym.py}
\end{longlisting}

The script creates a \texttt{results} directory in the current working directory and organizes data in a \texttt{<trial\-name>\/<phantom>\/<target>\/<model>} structure. Each model folder contains:

\begin{itemize}
	\item \texttt{eval}: Trajectory data from policy evaluation.
	\item \texttt{models}: Saved PyTorch models.
	\item \texttt{logs}: Tensorboard logs.
\end{itemize}

\subsubsection{Mesh Processing}
To use a custom aorta, perform a V-HACD convex decomposition. A tool called \texttt{stl2mjcf} is available at \url{https://github.com/tudorjnu/stl2mjcf}. To install:

\begin{minted}{bash}
pip install git+git@github.com:tudorjnu/stl2mjcf.git
\end{minted}

After installation, use \texttt{stl2mjcf --help} to see the available commands. Add the resulting XML file to \texttt{cathsim/assets} and the meshes folder to \texttt{cathsim/assets/meshes/}. (You may need to adjust V-HACD parameters for best results.)

\subsubsection{Adding Elements}

\paragraph{Adding a Phantom.} After processing your mesh (see Mesh Processing), add the files to \texttt{src/cathsim/dm/components/phantom\_assets/}. For example, if your phantom is named \texttt{my\_phantom.xml}, you can select it in your code as follows:

\begin{minted}{python}
import cathsim.gym.envs
import gymnasium as gym

task_kwargs = dict(
    phantom="my_phantom",
    target=[0.1, 0.1, 0.1],  # select a target based on the mesh or embed it into the xml
)

env = gym.make("cathsim/CathSim-v0", **task_kwargs)
\end{minted}

For more control, you can manually set up the aorta using the \texttt{mjcf} interface. A more detailed example:

\begin{minted}{python}
from cathsim.gym.envs import CathSim

phantom = MyPhantom()
tip = Tip(n_bodies=4)
guidewire = Guidewire(n_bodies=80)
task = Navigate(
    phantom=phantom,
    guidewire=guidewire,
    tip=tip,
    target=target,
    **kwargs,
)
env = composer.Environment(
    task=task,
    random_state=random_state,
    strip_singleton_obs_buffer_dim=True,
)

env = CathSim(dm_env=env)
\end{minted}

\paragraph{Adding a Guidewire.} A guidewire can be created similarly to the phantom and then integrated into the task. For further details on using \texttt{mjcf}, see \url{https://github.com/google-deepmind/dm_control/tree/main/dm_control/mjcf}.

\subsubsection{Terms of Use}
Please review the project’s \texttt{TERMS.md} before using the software.

\subsubsection{License}
The work is free to copy, distribute, display, perform, or remix for non-commercial purposes only.

% % --- Example Code Listings Section ---
% \section{Code Listings}
%
% \subsection{CathSim Code Sample}
% \begin{quote}
% 	The GitHub repository at \url{https://github.com/airvlab/cathsim} contains the simulator code.
% \end{quote}
%
% \begin{longlisting}
% 	\mycaption{CathSim as Gym Environment}{Demonstration of how CathSim can be used as a Gym environment.}
% 	\label{lst:cathsim-env}\inputminted[firstline=1]{python}{postamble/appendices/cathsim/quickstart.py}
% \end{longlisting}
%
% \begin{longlisting}
% 	\mycaption{CathSim Integration with RL Frameworks}{Demonstration of how CathSim can be integrated with RL frameworks.}
% 	\label{lst:cathsim-rl-training}\inputminted[firstline=1]{python}{postamble/appendices/cathsim/rl_compatibility.py}
% \end{longlisting}


==> postamble/appendices/code/main.tex <==
\section{Code Listings}

\subimport{cathsim}{main.tex}



==> postamble/appendices/copyrights.tex <==
\section{Copyright and Reuse Permissions}

Parts of this thesis are based on the author’s previously published work listed below. According to the reuse policies of respective publishers, including Springer Nature and IEEE, authors are permitted to reuse their published material in their thesis or dissertation, provided that proper citation and acknowledgment are included.

\vspace{1em}

\textbf{Springer Nature:} Material from Springer Nature publications is reused in accordance with their author rights policy, which allows reuse of the Version of Record in theses and dissertations. The following acknowledgment applies to all Springer Nature content: \emph{"Reproduced with permission from Springer Nature."}

\vspace{1em}

\textbf{IEEE:} Material from IEEE publications is reused in accordance with IEEE's author rights guidelines, which allow reuse in theses and dissertations under the condition that appropriate copyright notices are included. The IEEE copyright notice ``\emph{\copyright 2024 IEEE. Reprinted, with permission, from [full citation].}'' is provided with any reused material from IEEE publications.

\vspace{1em}

When this thesis is made publicly available, the following notice applies in reference to IEEE copyrighted material:

\begin{quote}
	``In reference to IEEE copyrighted material which is used with permission in this thesis, the IEEE does not endorse any of University of Liverpool products or services. Internal or personal use of this material is permitted. If interested in reprinting/republishing IEEE copyrighted material for advertising or promotional purposes or for creating new collective works for resale or redistribution, please go to \url{http://www.ieee.org/publications_standards/publications/rights/rights_link.html} to learn how to obtain a License from RightsLink. If applicable, University Microfilms and/or ProQuest Library, or the Archives of Canada may supply single copies of the dissertation.''
\end{quote}


\paragraph{Publications Reused in This Thesis:}


\begin{enumerate}
	\item \textbf{Tudor Jianu}, Baoru Huang, Minh Nhat Vu, Mohamed E.M.K. Abdelaziz, Sebastiano Fichera, Chun-Yi Lee, Pierre Berthet-Rayne, Ferdinando Rodriguez y Baena, Anh Nguyen. (2024). \emph{CathSim: An Open-source Simulator for Endovascular Intervention}. \emph{IEEE Transactions on Medical Robotics and Bionics}. IEEE.
	      \emph{\copyright 2024 IEEE. Reprinted, with permission, from the original publication.}

	\item \textbf{Tudor Jianu}, Baoru Huang, Hoan Nguyen, Pierre Berthet-Rayne, Sebastiano Fichera, Anh Nguyen. (2024). \emph{DeepWire: Spherical Coordinate-Based Deep Learning for Accurate Guidewire Shape Reconstruction}. In \emph{Proceedings of the 9th International Conference on Biomedical Signal and Image Processing (ICBIP 2024)}, Suzhou, China.
	      \emph{\copyright 2024 IEEE. Reprinted, with permission, from the original publication.}

	\item \textbf{Tudor Jianu}, Baoru Huang, Pierre Berthet-Rayne, Sebastiano Fichera, Anh Nguyen. (2023). \emph{3D Guidewire Shape Reconstruction from Monoplane Fluoroscopic Images}. \emph{International Conference on Robot Intelligence Technology and Applications}, pp. 84--94. Springer.\\
	      \emph{Reproduced with permission from Springer Nature.}

	\item \textbf{Tudor Jianu}, Baoru Huang, Pierre Berthet-Rayne, Sebastiano Fichera, Anh Nguyen. (2023). \emph{3D Guidewire Shape Reconstruction from Monoplane Fluoroscopic Images}. \emph{11th International Conference on Robot Intelligence Technology and Applications (RiTA)}, 2023.
	      \emph{Reproduced with permission from Springer Nature.}
\end{enumerate}


% \subsection{Additional Related Publications}
%
% \begin{enumerate}
% 	\setcounter{enumi}{2}
% 	\item \textbf{Tudor Jianu}, Baoru Huang, Tuan Vo, Minh Nhat Vu, Jingxuan Kang, Hoan Nguyen, Olatunji Omisore, Pierre Berthet-Rayne, Sebastiano Fichera, Anh Nguyen. (2024). \emph{Autonomous Catheterization with Open-source Simulator and Expert Trajectory}. - [Manuscript/Preprint status depending on final publication].
%
% 	\item Jingxuan Kang, \textbf{Tudor Jianu}, Baoru Huang, Binod Bhattarai, Ngan Le, Frans Coenen, Anh Nguyen. (2023). \emph{Translating Simulation Images to X-ray Images via Multi-Scale Semantic Matching}. arXiv. [Open Access].
% \end{enumerate}


All content reused from published sources is cited appropriately throughout the thesis. Any figures, tables, or excerpts are accompanied by the necessary copyright acknowledgments in their captions or associated text.


==> postamble/appendices/extra_aortas.tex <==
\section{Additional Aortic Models in CathSim}

In addition to Type-I Aortic Arch model which is mainly used in our experiments, we incorporate three distinct aortic models to enrich our anatomical dataset. These models include a high-fidelity Type-II aortic arch and a Type-I aortic arch with an aneurysm, both sourced from Elastrat, Switzerland. Furthermore, a low tortuosity aorta model, based on a patient-specific CT scan, is included. With these three additional representations, our simulator contains four distinct aorta models. These models aim to enhance the diversity and accuracy of aortic structures available for research and educational endeavors. These aortas are visualized in Fig.~\ref{fig:three aorta}.

\begin{figure}[ht]
	\centering
	\subfloat[Type-I (Aneurysm)]{\includegraphics[width=0.3\textwidth]{assets/aortas/aneurysm.png}}
	\hfill
	\subfloat[Type-II]{\includegraphics[width=0.3\textwidth]{assets/aortas/type2.png}}
	\hfill
	\subfloat[Low Tortuosity]{\includegraphics[width=0.3\textwidth]{assets/aortas/low_tort.png}}
	\caption{Aortic Models.}
	\label{fig:three aorta}
\end{figure}


==> postamble/appendices/network_choice.tex <==
\section{Network Choice}\label{app:network-choice}

In our experimental trials, we implemented a transformer-based architecture, drawing inspiration from the visual transformer by~\autocite{dosovitskiy2020image}. This architecture was specifically tailored with an image size of \(80\), a patch size of \(10\), and a single-channel configuration, alongside a depth of \(3\) and \(4\) heads within the attention layers. Despite these specifications, the transformer model did not achieve the expected performance level in our specialized domain of endovascular navigation. It notably struggled to complete the designated tasks within the desired timeframe. This underperformance, coupled with signs of convergence, is illustrated in Fig~\ref{app-fig:vit}, highlighting the challenges encountered in applying this model to our specific context.

\begin{figure}[h]
	\centering
	\includegraphics{assets/rebuttal/vit.png}
	\caption{\textbf{ViT-Based ENN Trials:} Initial results indicate that using ViT as a feature extractor does not improve outcomes and fails to meet the target within the time limit, despite showing convergence.}
	\label{app-fig:vit}
\end{figure}


==> postamble/appendices/sim2real.tex <==
\section{Sim-to-Real Imaging Gap}

We showcase the adaptability of our endovascular simulator using domain adaptation techniques. This is crucial for translating simulated environments into more realistic, X-ray-like images. The implementation of this approach is based on the work of~\autocite{kang2024translating}. Their method, employing multi-scale semantic matching, effectively ensures the preservation of essential structural information in medical images while transitioning from simulated to real-world imaging styles. This technique has demonstrated significant success in producing realistic X-ray images and has set a new benchmark in the field. For an in-depth understanding and visual representation of this adaptation process, we refer readers to the detailed findings and illustrations in the work of~\autocite{kang2024translating}. The adapted images can be visualized in Fig.~\ref{app-fig:sim2real}.

\begin{figure}[h]
	\centering
	\subfloat[]{\includegraphics[width=0.28\linewidth, height=0.28\linewidth]{assets/sim2real/0.png}}
	\hspace{1px}
	\subfloat[]{\includegraphics[width=0.28\linewidth, height=0.28\linewidth]{assets/sim2real/1.png}}
	\hspace{1px}
	\subfloat[]{\includegraphics[width=0.28\linewidth, height=0.28\linewidth]{assets/sim2real/2.png}}
	\mycaption{Sim-to-Real Adaptation}{ Demonstration of sim-to-real domain adaptation for creating realistic renderings, featuring \textit{a)} the input image, \textit{b)} the resultant generated image, and \textit{c)} a real X-ray image example. Figure addapted from~\autocite{kang2024translating}}
	\label{app-fig:sim2real}
\end{figure}


==> postamble/appendices/speed_evaluation.tex <==
\section{CathSim Speed Evaluation}

\begin{sidebysidefigures}[.5]
	\begin{leftfigure}
		\adjustimage{left}{assets/episode_time.png}
		\captionof{figure}{CathSim training speed.}
		\label{app1fig:fps}
	\end{leftfigure}%
	\begin{rightfigure}
		\vspace{0.35cm}
		\input{tables/training_times_coparison.tex}
	\end{rightfigure}
\end{sidebysidefigures}


As illustrated in Fig.~\ref{app1fig:fps}, we provide a comparison of frames per second (FPS) for the various algorithms we employed during model training. It is evident that utilizing solely the internal state space, comprised of joint positions and velocities, facilitates expedited training processes. In contrast, integrating all modalities into the training process results in its deceleration. The most significant computational demand arises from the dual convolutional neural networks utilized in both the image and mask representations. However, despite this load, the algorithms exhibit respectable computational speed, even during the training phase. Our simulator supports approximately $40$ to $80$ frames per second performance for all implemented algorithms, underscoring the computational speed of our simulation environment. Moreover, we provide the training times in terms of hours for the different modalities in Table~\ref{app1tab:training-time}.


==> postamble/appendices/tables/training_times_coparison.tex <==
\captionof{table}{Comparative training times}\label{app1tab:training-time}
\begin{tabular}{l r r}
	\toprule
	\multirowcell{2}{\thead{Algorithm}} & \multicolumn{2}{c}{\thead{Training Time~(\(\mathbf{\unit{\hour}}\))}}                   \\
	\cmidrule{2-3}
	                                    & \thead{BCA}                                                           & \thead{LCCA}    \\
	\midrule
	Image                               & $3.00 \pm 0.11$                                                       & $2.54 \pm 0.17$ \\
	Image+Mask                          & $4.20 \pm 0.05$                                                       & $4.60 \pm 1.29$ \\
	Internal                            & $2.38 \pm 0.15$                                                       & $2.20 \pm 0.18$ \\
	Internal+Image                      & $3.15 \pm 0.28$                                                       & $3.54 \pm 0.29$ \\
	\textbf{ENN}                        & $4.61 \pm 0.22$                                                       & $4.83 \pm 0.41$ \\
	\bottomrule
\end{tabular}


==> postamble/appendices/traditional_path_planning.tex <==
\section{Traditional Path Planning}

To emphasize our choice of using a neural network policy as the expert, we conducted a defining experiment. We initially used the A* planner~\autocite{hart1968formal} to identify the most straightforward route from a starting position to the goal, ensuring sampling was restricted to the aortic arch. This plan is depicted in Fig.~\ref{appfig:path-planning}. However, the results revealed that the shortest path is not always the best. The cannulation efficiency along this route was suboptimal, and there was no standardized method to determine the exact actuation for the guidewire tip to follow this path. Expanding our research, we utilized a Multilayer Perceptron (MLP) to predict the next action from a sequence of observations. Yet, this model also faced difficulties in following the desired route, highlighting the intrinsic complexities of the task. The agent's actual path, showing the guidewire's deviation, can be seen below:

\begin{figure}[h]
	\centering
	\includegraphics{assets/path_following.png}
	\caption{Path Planning}
	\label{appfig:path-planning}
\end{figure}


==> preamble/copyright.tex <==
\clearpage
\chapter*{Copyright}

\onehalfspacing
The University will have a standardized copyright notice. You should write it here.
\clearpage

